Dissecting the impact of different loss functions with gradient surgery

Pair-wise loss is an approach to metric learning that learns a semantic embedding by optimizing a loss function that encourages images from the same semantic class to be mapped closer than images from different classes. The literature reports a large and growing set of variations of the pair-wise loss strategies. Here we decompose the gradient of these loss functions into components that relate to how they push the relative feature positions of the anchor-positive and anchor-negative pairs. This decomposition allows the unification of a large collection of current pair-wise loss functions. Additionally, explicitly constructing pair-wise gradient updates to separate out these effects gives insights into which have the biggest impact, and leads to a simple algorithm that beats the state of the art for image retrieval on the CAR, CUB and Stanford Online products datasets.

==> figure/GD_res.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figure/GD.jpg}
    \caption{Comparison on different gradient direction on CUB, CAR, SOP and In-shop dataset}
    \label{fig:result_gd}
\end{figure}

==> table/exp_grad_temp.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{c|c|cccc|cccc}
 \multicolumn{2}{c|}{Setting} & \multicolumn{4}{c|}{CAR} & \multicolumn{4}{c}{In-shop} \\
 \hline
$\tau$ & $w_t$ & lr 0.1 & lr 0.2 & lr 0.3 & lr 0.4 & lr 1.0 & lr 2.0 & lr 3.0 & lr 4.0 \\
\hline
0.1 & $w_t^{nca}$ & \cellcolor[HTML]{FFDC79}75.6 $\pm$ 0.8 & \cellcolor[HTML]{FFEFC0}71.8 $\pm$ 0.6 & \cellcolor[HTML]{FFF9E5}66.4 $\pm$ 1.6 & \cellcolor[HTML]{FFFFFF}62.5 $\pm$ 0.9 & \cellcolor[HTML]{FFECB6}87.4 $\pm$ 0.2 & \cellcolor[HTML]{FFEBB1}87.5 $\pm$ 0.2 & \cellcolor[HTML]{FFF1C7}87.1 $\pm$ 0.2 & \cellcolor[HTML]{FFF8E4}86.6 $\pm$ 0.3 \\
1 & $w_t^{nca}$ & \cellcolor[HTML]{FFDB75}75.8 $\pm$ 0.2 & \cellcolor[HTML]{FFE8A5}74.1 $\pm$ 0.6 & \cellcolor[HTML]{FFF0C4}71.2 $\pm$ 1.2 & \cellcolor[HTML]{FFF7E1}67.0 $\pm$ 0.5 & \cellcolor[HTML]{FFE7A5}87.7 $\pm$ 0.3 & \cellcolor[HTML]{FFE9A9}87.6 $\pm$ 0.2 & \cellcolor[HTML]{FFEAAF}87.5 $\pm$ 0.1 & \cellcolor[HTML]{FFF7DF}86.7 $\pm$ 0.5 \\
3 & $w_t^{nca}$ & \cellcolor[HTML]{FFDF84}75.3 $\pm$ 0.3 & \cellcolor[HTML]{FFD666}76.2 $\pm$ 0.3 & \cellcolor[HTML]{FFDC79}75.6 $\pm$ 0.8 & \cellcolor[HTML]{FFEAAD}73.9 $\pm$ 0.3 & \cellcolor[HTML]{FFDB78}88.3 $\pm$ 0.0 & \cellcolor[HTML]{FFD666}88.6 $\pm$ 0.1 & \cellcolor[HTML]{FFE08A}88.1 $\pm$ 0.5 & \cellcolor[HTML]{FFE291}88.0 $\pm$ 0.2 \\
10 & $w_t^{nca}$ & \cellcolor[HTML]{FFF3CF}69.6 $\pm$ 0.2 & \cellcolor[HTML]{FFEEBC}72.4 $\pm$ 0.5 & \cellcolor[HTML]{FFECB4}73.6 $\pm$ 0.4 & \cellcolor[HTML]{FFEBB1}73.7 $\pm$ 0.6 & \cellcolor[HTML]{FFFFFF}86.1 $\pm$ 0.2 & \cellcolor[HTML]{FFF0C5}87.1 $\pm$ 0.1 & \cellcolor[HTML]{FFF2CC}87.0 $\pm$ 0.2 & \cellcolor[HTML]{FFF8E3}86.6 $\pm$ 0.5 \\
\hline
$\tau$ & $w_t$ & lr 0.1 & lr 0.2 & lr 0.3 & lr 0.4 & lr 1.0 & lr 2.0 & lr 3.0 & lr 4.0 \\
\hline
0.1 & $w_t^{2nd}$ & \cellcolor[HTML]{FFDB76}75.6 $\pm$ 0.5 & \cellcolor[HTML]{FFEAAC}71.7 $\pm$ 0.5 & \cellcolor[HTML]{FFEEBE}66.7 $\pm$ 0.5 & \cellcolor[HTML]{FFF0C4}64.1 $\pm$ 0.6 & \cellcolor[HTML]{FFE7A1}87.3 $\pm$ 0.2 & \cellcolor[HTML]{FFE499}87.5 $\pm$ 0.3 & \cellcolor[HTML]{FFECB5}86.6 $\pm$ 0.1 & \cellcolor[HTML]{FFECB7}86.0 $\pm$ 0.2 \\
1 & $w_t^{2nd}$ & \cellcolor[HTML]{FFDB78}75.5 $\pm$ 0.3 & \cellcolor[HTML]{FFDD7F}75.0 $\pm$ 1.0 & \cellcolor[HTML]{FFE69F}72.6 $\pm$ 0.4 & \cellcolor[HTML]{FFECB5}70.6 $\pm$ 0.5 & \cellcolor[HTML]{FFE8A7}87.2 $\pm$ 0.3 & \cellcolor[HTML]{FFE498}87.5 $\pm$ 0.1 & \cellcolor[HTML]{FFE59C}87.4 $\pm$ 0.3 & \cellcolor[HTML]{FFECB4}86.8 $\pm$ 0.5 \\
3 & $w_t^{2nd}$ & \cellcolor[HTML]{FFECB7}69.6 $\pm$ 0.8 & \cellcolor[HTML]{FFDF87}74.4 $\pm$ 0.3 & \cellcolor[HTML]{FFDA72}75.9 $\pm$ 0.5 & \cellcolor[HTML]{FFD666}76.7 $\pm$ 0.4 & \cellcolor[HTML]{FFECB4}86.8 $\pm$ 0.2 & \cellcolor[HTML]{FFE089}87.8 $\pm$ 0.2 & \cellcolor[HTML]{FFD666}88.4 $\pm$ 0.1 & \cellcolor[HTML]{FFDA74}88.1 $\pm$ 0.1 \\
10 & $w_t^{2nd}$ & \cellcolor[HTML]{FFFFFF}38.3 $\pm$ 0.6 & \cellcolor[HTML]{FFFCF2}44.0 $\pm$ 1.1 & \cellcolor[HTML]{FFFAEC}46.8 $\pm$ 0.4 & \cellcolor[HTML]{FFF8E4}50.0 $\pm$ 0.6 & \cellcolor[HTML]{FFFFFF}63.9 $\pm$ 0.2 & \cellcolor[HTML]{FFFBEF}69.1 $\pm$ 0.4 & \cellcolor[HTML]{FFF9E6}71.7 $\pm$ 0.6 & \cellcolor[HTML]{FFF7E1}73.3 $\pm$ 0.2 \\

\hline
\end{tabular}
\caption{Experiments on comparing scaling parameters with various learning rates(lr). Recall@1 performance on CAR and In-shop dataset}
\label{table:grad_temp_CAR}
\end{table*}
